FreeST: Context-free Session Types in a Functional Language

FreeST is an experimental concurrent programming language. Based on a core linear functional programming language, it features primitives to fork new threads, and for channel creation and communication. A powerful type system of context-free session types governs the interaction on channels. The compiler builds on a novel algorithm for deciding type equivalence of context-free session types. This abstract provides a gentle introduction to the language and discusses the validation process and runtime system.

==> eptcsdata.tex <==
\providecommand{\firstpage}{12}
\providecommand{\publicationstatus}{F. Martins, D. Orchard (Eds.): Programming Language Approaches \\
to Concurrency- \& Communication-cEntric Software (PLACES 2019)\\
EPTCS 291, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.291.2}{10.4204/EPTCS.291.2}}
\pdfoutput=1

